Presentation and Publication: Loss and Slippage in Networks of Automated Market Makers

Automated market makers (AMMs) are smart contracts that automatically trade electronic assets according to a mathematical formula. This paper investigates how an AMM's formula affects the interests of liquidity providers, who endow the AMM with assets, and traders, who exchange one asset for another at the AMM's rates. *Linear slippage* measures how a trade's size affects the trader's return, *angular slippage* measures how a trade's size affects the subsequent market price, *divergence loss* measures the opportunity cost of providers' investments, and *load* balances the costs to traders and providers. We give formal definitions for these costs, show that they obey certain conservation laws: these costs can be shifted around but never fully eliminated. We analyze how these costs behave under *composition*, when simple individual AMMs are linked to form more complex networks of AMMs.

==> arbitrage.tex <==
In the case where the AMM serves as the truth for the current exchange rate (via arbitrage), we want to be able to adjust AMMs to do damage control.
Namely, in this section we outline a minimal set of constraints any time-varying AMM should satisfy and describe methods for reducing loss and slippage.

\subsection{Necessary Constraints}

Suppose we have an AMM $f$ and we want to transform this AMM into another AMM $\tilde{f}$ to the benifit say of traders or liquidity providers.
What basic requirements should we impose on $\tilde{f}$ that relate it back to $f$?

Up to this point we have assumed agents interact with AMM contracts in two ways:
\begin{itemize}
    \item $Trade(x,\delta)$ which updates $x \to x + \delta,f(x) \to f(x + \delta)$ \\
    ($\delta > 0 $)
    \item $Deposit/Withdraw(\delta_x,\delta_y)$ which updates $x \to x + \delta_x,y \to y + \delta_y$ \\ ($\delta_x,\delta_y > 0$ or $\delta_x,\delta_y < 0$)
\end{itemize}

Implicit to the use of the operations is that reserves can only change when providers or traders interact with the contract.


If we introduce a new operation $\textit{Adjust}$ which transforms $f \to \tilde{f}$, we can understand how it must be constrained by thinking about how it interacts with the previous two mentioned operations.

It really only makes since for $Adjust$ to be called after a call to $Trade$ since that is when new information has been provided that will tell $Adjust$ how to modify the original curve.
So suppose $Adjust$ follows the execution of one some $Trade$ call which ended in state $(x,f(x))$.
Because $Adjust$ is an operation requiring no input from providers or traders, it should not be allowed to change the current reserves.
Namely, after $Adjust$, the new state must be $(x,\tilde{f}(x))$ where $\tilde{f}(x) = f(x)$.
So any such $Adjust$ operation must preserve the current state.

Secondly, suppose $Adjust$ were to change the current exchange rate.
If $Adjust$ was called after a call to $Trade(x,\delta)$ for small $\delta > 0$, then a trader could launch an arbitrage attack.
($\delta$ small enough so $f'(x) \approx f'(x + \delta)$)
Namely say $f'(x+ \delta) \neq \tilde{f}'(x + \delta)$ and wlog that $\tilde{f}'(x + \delta) > f'(x + \delta)$.
A trader knowing this $Adjust$ call would eventually occur could do the following:
They could run $Trade(x,\delta)$ to get roughly $-\delta f'(x + \delta)$ in asset $Y$.
Say the new state after this $Trade$ call would be the stable state so the trader couldn't extract any more profit.
If after $Adjust$ they did a $Y \to X$ trade then they would get $\frac{-\delta f'(x + \delta)}{-\delta \tilde{f}'(x + \delta)} = \frac{f'(x + \delta)}{\tilde{f}(x + \delta)} > 1$ of $X$ in return.
A symmetric argument shows $\tilde{f}'(x + \delta) \not < f'(x + \delta)$.
In either case a trader can get a risk-free profit, so we must require $\tilde{f}'(x + \delta) = f'(x + \delta)$.

Thus any $Adjust$ operation must preserve the current state and the current exchange rate.

\subsection{Optimal AMMs}

The previous section tells us that if we are to transform some $f \to \tilde{f}$, if the state is $(x,f(x))$, then the resulting state in the new AMM $\tilde{f}$ is $(x,\tilde{f}(x))$ where $f(x) = \tilde{f(x)}$ and $f'(x) = \tilde{f}'(x)$.
This section aims to determine exactly how much we can modify an AMM in order to minimize the expected cost associated with it.

Say we have an AMM $A$ in state $(x_0,f(x_0))$ where $f'(x_0) = \frac{-v}{1 - v}$.
If we were to completely flatten the AMM around this point by taking it's linear approximation, we could conceivably reduce angular slippage to $0$ and so it follows from Equation \ref{cost_angular} that the cost would also be $0$ near $\phi(\bv)$.
The resulting linear approximation is not an AMM according to our definition.
However, as we will see it is a useful tool for formulating a notion of optimality for an AMM.
The linear approximation is given by the equation
\begin{align*}
    y(x) = f'(x)(x - x_0) + f(x_0)
\end{align*}
which intersects the $x$-axis at $x^{*} = x_0 - \frac{f(x_0)}{f'(x_0)}$ and the $y$-axis at $y^{*} = -f'(x_0)x_0 + f(x_0)$.
In this linear case, $\bv'$ only has three possible values: $\bv,(0,1),(1,0)$.
When $x_0 \leq x < x^{*}$ or $f(x_0) \leq y < y^{*}$, the corresponding valuation is $\bv$ so we get
\begin{align*}
    &C^Y_{\bv}(\bv';A) = C^Y_{\bv}(\bv;A) = 0 \\
    &C^X_{\bv}(\bv';A) =  C^X_{\bv}(\bv;A) = 0
\end{align*}

However when $x \geq x^{*}$ the $Y$ cost is
\begin{align*}
    &C^Y_{\bv}((0,1);A) = \frac{(1 - (1-v))}{1 - v}(x^{*} - x_0) \\
    &= \frac{v}{1 -v}(x_0 - \frac{f(x_0)}{f'(x_0)} - x_0) \\
    &=f(x_0)\frac{v}{1 - v}(\frac{1 - v}{v}) = f(x_0)  
\end{align*}

and similarly when $y > y^{*}$, the $X$ cost is
\begin{align*}
    &C^X_{\bv}((1,0);A) = \frac{(v - 1)}{v}(y^{*} - f(x_0)) \\
    &= C^X_{\bv}((1,0);A) = \frac{(v - 1)}{v}(-f'(x_0)x_0 + f(x_0) - f(x_0)) \\
    &= x_0\frac{(v - 1)}{v}(\frac{v}{1 - v}) = x_0 
\end{align*}

Returning then to our definition from Equation \ref{expected_cost} of expected cost, we get
\begin{align*}
    &E_p[C_{\bv}(\bv';A)] = \int_0^{v}p(\bv')C^Y_{\bv}(\bv';A)dv' + \int_v^{1}p(\bv')C^X_{\bv}(\bv';A)dv' \\
    &= \int_0^vp(\bv')y_0dv' + \int_v^1p(\bv')x_0dv' \\
    &= y_0\int_0^vp(\bv')dv' + x_0\int_v^1p(\bv')dv' \\
    &= y_0P(v' < v) + x_0P(v' >  v)
\end{align*}
This result has a very natural economic meaning.
For a linear AMM, if the market changes so that $v' < v$, then via arbitrage traders will be encouraged to drain reserves of asset $Y$ by an amount $y_0$.
In the reverse direction, if $v' > v$, then arbitrage traders will drain $x_0$ type $X$ assets from the reserves.
The above expression is what a linear AMM can expect to lose in value depending on what direction we expect the market to move.

In practice we wouldn't want to use a linear AMM but the expected cost of a linear AMM provides a useful benchmark for modifying AMMs.

\begin{theorem}
\end{theorem}

==> general_comp.tex <==
When talking about how composition relate to loss and slippage, it is useful to imagine our previous versions of composition upgraded to support simple linear markets as well.
If $A$ is an AMM, and $0 < r < 1$, this allows us to make sense of things like $A \oplus r,r \oplus A,r || A,A || r$.
Also, it might be useful to define a version of composition for AMMs where some of the reserves are inaccessible as in Uniswap V3.
This would allow us to say under this alternative version of composition constant-product AMMs are closed. 

\subsection{Unary Operators}
Things like: virtualization,projection, oracle adjustment operation.

\subsection{Binary Operators}
Things like: parallel,sequential composition.
